Media Accessibility Policy in Theory and Reality: Empirical Outreach to Audio Description Users in the United States

Audio description, a form of trans-modal media translation, allows people who are blind or visually impaired access to visually-oriented, socio-cultural, or historical public discourse alike. Although audio description has gained more prominence in media policy and research lately, it rarely has been studied empirically. Yet this paper presents quantitative and qualitative survey data on its challenges and opportunities, through the analysis of responses from 483 participants in a national sample, with 334 of these respondents being blind. Our results give insight into audio description use in broadcast TV, streaming services, for physical media, such as DVDs, and in movie theaters. We further discover a multiplicity of barriers and hindrances which prevent a better adoption and larger proliferation of audio description. In our discussion, we present a possible answer to these problems - the UniDescription Project - a media ecosystem for the creation, curation, and dissemination of audio description for multiple media platforms.

==> hicss51-packages.tex <==
\usepackage[letterpaper]{geometry}
\usepackage{hicss51}
\usepackage{times}
\usepackage[none]{hyphenat}
\usepackage{url}
\usepackage{latexsym}
\usepackage{minted}
\usepackage{indentfirst}
\usepackage{graphicx}
\graphicspath{{images/}}

